Kernel-based Generative Learning in Distortion Feature Space

This paper presents a novel kernel-based generative classifier which is defined in a distortion subspace using polynomial series expansion, named Kernel-Distortion (KD) classifier. An iterative kernel selection algorithm is developed to steadily improve classification performance by repeatedly removing and adding kernels. The experimental results on character recognition application not only show that the proposed generative classifier performs better than many existing classifiers, but also illustrate that it has different recognition capability compared to the state-of-the-art discriminative classifier - deep belief network. The recognition diversity indicates that a hybrid combination of the proposed generative classifier and the discriminative classifier could further improve the classification performance. Two hybrid combination methods, cascading and stacking, have been implemented to verify the diversity and the improvement of the proposed classifier.

==> Macros.tex <==
\newcommand{\refs}{\section*{References}
                  \markright{\MakeUppercase{References}}}
\newcommand{\probs}{\section*{Problems}
                   \markright{\MakeUppercase{Problems}}}
\newcounter{appcount}
\setcounter{appcount}{0}
\newcommand{\appendicesname}
            {Appendix\ \thechapter  \Alph{appcount}}
\newcommand{\bookappendicesname}
            {Appendix\ \Alph{appcount}}
\newcommand{\chapterappendix}[1]
          {\par\setcounter{section}{0}
           \setcounter{equation}{0}
           \setcounter{table}{0}
           \setcounter{figure}{0}
          \addtocounter{appcount}{1}   \renewcommand{\theequation}{\thechapter\Alph{appcount}.\arabic{equation}}
          \renewcommand{\thetable}{\thechapter\Alph{appcount}.\arabic{table}}
          \renewcommand{\thefigure}{\thechapter\Alph{appcount}.\arabic{figure}}
           \setcounter{section}{\arabic{chapter}\Alph{section}}
           \if@openright\cleardoublepage\else\clearpage\fi
           \chapter*{\huge{\appendicesname}\newline\newline \Huge{#1}}
           \addcontentsline{toc}{section}{\thechapter\Alph{appcount} #1}
           \markright{\MakeUppercase{\appendicesname.\ { #1}}}}
\newcommand{\bookappendix}[1]
          {\par\setcounter{section}{0}
           \setcounter{equation}{0}
           \setcounter{table}{0}
           \setcounter{figure}{0}
          \addtocounter{appcount}{1}   \renewcommand{\theequation}{\Alph{appcount}.\arabic{equation}}
           \renewcommand{\thetable}{\Alph{appcount}.\arabic{table}}
             \renewcommand{\thefigure}{\Alph{appcount}.\arabic{figure}}
           \setcounter{section}{\arabic{chapter}\Alph{section}}
           \if@openright\cleardoublepage\else\clearpage\fi
           \chapter*{\huge{\bookappendicesname}\newline\newline \Huge{#1}}
           \addcontentsline{toc}{chapter}{\bookappendicesname #1}
          \markright{\MakeUppercase{\bookappendicesname.\ { #1}}} }
\newcounter{example}
\setcounter{example}{0}
\newcounter{property}
\setcounter{property}{0}
\newcommand{\caution}
{\begin{picture}(32,26)(0,5)
\thicklines
\drawpath{16.0}{22.0}{4.0}{4.0}
\drawpath{4.0}{4.0}{24.0}{4.0}
\drawpath{24.0}{4.0}{22.0}{4.0}
\drawpath{24.0}{4.0}{28.0}{4.0}
\drawpath{28.0}{4.0}{16.0}{22.0}
\thinlines
\drawthickdot{14.0}{6.0}
\drawthickdot{18.0}{6.0}
\Thicklines
\drawpath{14.0}{16.0}{14.0}{8.0}
\drawpath{18.0}{16.0}{18.0}{8.0}
\end{picture}}
\newcommand{\placefigone}[6]{
\begin{figure}[h!]
\begin{center}
\psfrag{#1}{\small{#2}}
\psfrag{#3}{\small{#4}}
\includegraphics*[scale=0.75]{#5}
\end{center}
\caption{#6}
\end{figure}}
\newcommand{\placefigonetitle}[8]{
\begin{figure}[h!]
\begin{center}
\psfrag{#1}{\small{#2}}
\psfrag{#3}{\small{#4}}
\psfrag{#5}{\small{#6}}
\includegraphics*[scale=0.75]{#7}
\end{center}
\caption{#8}
\end{figure}}
\newcommand{\msp}[1]{{\phantom{\mbox{#1}}}}
\newcommand{\mvsp}[1]{\rule{0in}{#1in}}
\newcommand{\bc}[1]{\vspace{11pt}\par\noindent\caution\hspace{11pt}{\bf
#1}\vspace{11pt}\par\noindent}
\newcommand{\ec}{\par\noindent\hfill \caution\par\noindent}
\newcommand{\be}{\[}
\newcommand{\ee}{\]}
\newcommand{\ben}{\begin{equation}}
\newcommand{\een}{\end{equation}}
\newcommand{\bea}{\begin{eqnarray*}}
\newcommand{\eea}{\end{eqnarray*}}
\newcommand{\bean}{\begin{eqnarray}}
\newcommand{\eean}{\end{eqnarray}}
\newcommand{\bex}[1]{\addtocounter{example}{1}\vspace{4pt}\par\noindent{\bf Example
\thechapter.\theexample\ -- \
#1}\vspace{1pt}\par\noindent}
\newcommand{\eex}{\par\noindent\hfill $\diamondsuit$\par\noindent}
\newcommand{\bep}[1]{\addtocounter{property}{1}\vspace{4pt}\par\noindent{\bf Property
\thechapter.\theproperty\ -- \
#1}\vspace{1pt}\par\noindent}
\newcommand{\eep}{\par\noindent\hfill $\square$\par\noindent}
\newcommand{\dis}{\displaystyle}
\newcommand{\mat}[4]{\left[\begin{array}{cc}{#1}&{#2}\\
{#3}&{#4}\end{array}\right]}
\newcommand{\mata}[4]{\begin{array}{cc}{#1}&{#2}\\
{#3}&{#4}\end{array}}
%\newtheorem{theorem}{Theorem}[section]
\newcommand{\et}{\par\noindent\hfill $\triangle$\par\noindent}
%\newtheorem{lemma}{Lemma}[section] %with [section] it will number the lemma in the section
%\newtheorem{lemma}{Lemma}
%\newtheorem{prop}{Proposition}[section]
\newcommand{\vvec}[2]{\left[\begin{array}{c}{#1}\\ [0.1 truein]{#2}\end{array}\right]}
\newcommand{\vvecc}[3]{\left[\begin{array}{c}{#1}\\ [0.1 truein]{#2}\\ [0.1
truein]{#3}\end{array}\right]}
\newcommand{\vvecr}[2]{\left[\begin{array}{cc}{#1}&{#2}\end{array}\right]}
\newcommand{\vveccr}[3]{\left[\begin{array}{ccc}{#1}&{#2}&{#3}\end{array}\right]}
\newcommand{\note}[1]{\marginpar{{\bf {#1}}}}
\newcommand{\see}{{\it see} }
\newcommand{\ind}{$\phantom{xx}$}
%
\newcommand{\cov}{\mbox{cov}}
\newcommand{\covth}{{\bf C}_{\thh}}
\newcommand{\dat}{n=0,1,\ldots,N-1}
\newcommand{\diag}{{\rm diag}}
\newcommand{\dlp}[2]{\frac{\partial\ln p({\bf x};{#1})}{\partial {#2}}}
\newcommand{\ddlp}[2]
{\frac{\partial^2\ln p({\bf x};{#1})}{\partial {#2}^2}}
\newcommand{\dlpxn}[2]{\frac{\partial\ln p(\x;{#1})}{\partial {#2}}}
\newcommand{\ddlpxn}[2]
{\frac{\partial^2\ln p(\x;{#1})}{\partial {#2}^2}}
\newcommand{\ddlpp}[3]{\frac{\partial^2\ln p({\bf x};{#1})}{\partial {#2}
\partial {#3}}}
\newcommand{\dxy}{dx\,dy}
\newcommand{\gauss}{\frac{1}{(2\pi\s)^\frac{N}{2}}}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\halfsm}{\textstyle{\frac{1}{2}}}
\newcommand{\HH}{{\cal H}}
\newcommand{\Ho}{{\cal H}_0}
\newcommand{\Hl}{{\cal H}_1}
\newcommand{\intt}{\int_{-\half}^\half}
\newcommand{\intinf}{\int_{-\infty}^\infty}
\newcommand{\intint}{\int\hspace{-0.075in}\int}
\newcommand{\jj}{j2\pi f}
\newcommand{\Jm}{J_{{\rm min}}}
\newcommand{\Jmk}{J_{{\rm min}_k}}
\newcommand{\ninf}{-\infty<n<\infty}
\newcommand{\pmfN}{p_{X_1,X_2,\ldots,X_N}[x_1,x_2,\ldots,x_N]}
\newcommand{\p}[1]{p({\bf x};{#1})}
\newcommand{\pB}[1]{p({\bf x}|{#1})}
\newcommand{\pn}{\pi f_0n}
\newcommand{\pr}{\partial}
\newcommand{\PP}[1]{P_{xx}(f;{#1})}
\newcommand{\PPt}{P_{\tilde{x}\tilde{x}}(f)}
\newcommand{\pxy}{p_{X,Y}(x,y)}
\newcommand{\pxn}{p_{X_1,X_2,\ldots,X_N}(x_1,x_2,\ldots,x_N)}
\newcommand{\pxN}{p_{X_1,X_2,\ldots,X_N}(x_1,x_2,\ldots,x_N)dx_1\,dx_2\ldots dx_N}
\newcommand{\rxx}{r_{xx}[}
\newcommand{\rxy}{r_{X,Y}[}
\newcommand{\rt}{r_{\xt\xt}[}
\newcommand{\s}{\sigma^2}
\newcommand{\samp}{{\cal S} }
\newcommand{\sampele}{{\scriptstyle{\cal S}}}
\newcommand{\sm}{$\boldsymbol{ \smile^{\phantom{a}^{\hspace{-0.21in}.\,.}}}$ }
\newcommand{\smiley}{(\hspace{-0.02in}${\phantom{.}\atop\mbox{\sm}}$\hspace{-0.035in})}
\newcommand{\sn}{s[n]}
\newcommand{\SSN}{\sum_{n=0}^{N-1}}
\newcommand{\SSM}{\sum_{n=-M}^M}
\newcommand{\tworeg}[5]{#1=\left\{\begin{array}{ll}#2&#3\\ #4&#5\end{array}\right.}
\newcommand{\tho}{\theta}
\newcommand{\tr}{\mbox{tr}}
\newcommand{\vv}{\mbox{var}}
\newcommand{\x}{x[n]}
\newcommand{\xs}{{x_1,x_2,\ldots,x_N}}
\newcommand{\Xs}{{X_1,X_2,\ldots,X_N}}
\newcommand{\w}{w[n]}
%
\newcommand{\alphh}{\hat{\alpha}}
\newcommand{\Ah}{\hat{A}}
\newcommand{\bfah}{\hat{{\bf a}}}
\newcommand{\bfbh}{\hat{{\bf b}}}
\newcommand{\At}{{\tilde{A}}}
\newcommand{\E}{{\cal E}}
\newcommand{\fh}{\hat{f}}
\newcommand{\calA}{{\cal A}}
\newcommand{\calB}{{\cal B}}
\newcommand{\calE}{{\cal E}}
\newcommand{\calX}{{\cal X}}
\newcommand{\calY}{{\cal Y}}
\newcommand{\calH}{{\cal H}}
\newcommand{\calP}{{\cal P}}
\newcommand{\calZ}{{\cal Z}}
\newcommand{\CN}{{\cal CN}}
\newcommand{\hht}{\tilde{h}}
\newcommand{\N}{{\cal N}}
\newcommand{\mut}{\tilde{\mu}}
\newcommand{\omt}{\tilde{\omega}}
\newcommand{\sh}{\hat{s}}
\newcommand{\ssh}[1]{\hat{\sigma^2_#1}}
\newcommand{\st}{\tilde{s}}
\newcommand{\thc}{\check{\theta}}
\newcommand{\thh}{{\hat{\theta}}}
\newcommand{\xt}{{\tilde{x}}}
\newcommand{\wt}{\tilde{w}}
\newcommand{\yt}{\tilde{y}}
\newcommand{\zt}{\tilde{z}}
%
\newcommand{\bfalph}{\mbox{\boldmath{$\alpha$}}}
\newcommand{\bfbeta}{\mbox{\boldmath{$\beta$}}}
\newcommand{\bfeps}{\mbox{\boldmath{$\epsilon$}}}
\newcommand{\bfeta}{\mbox{\boldmath{$\eta$}}}
\newcommand{\bfetah}{\hat{\mbox{\boldmath{$\eta$}}}}
\newcommand{\bfgamma}{\mbox{\boldmath{$\gamma$}}}
\newcommand{\bflamb}{\mbox{\boldmath{$\lambda$}}}
\newcommand{\bfLamb}{\mbox{\boldmath{$\Lambda$}}}
\newcommand{\bfmu}{\mbox{\boldmath{$\mu$}}}
\newcommand{\bfmut}{\tilde{\mbox{\boldmath{$\mu$}}}}
\newcommand{\bfomega}{\mbox{\boldmath{$\omega$}}}
\newcommand{\bfomt}{\tilde{\bfomega}}
\newcommand{\bfphi}{\mbox{\boldmath{$\phi$}}}
\newcommand{\bfpi}{\mbox{\boldmath{$\pi$}}}
\newcommand{\bfSig}{{\bf \Sigma}}
\newcommand{\bfth}{\mbox{\boldmath{$\theta$}}}
\newcommand{\bfTh}{\mbox{\boldmath{$\Theta$}}}
\newcommand{\bfthh}{\hat{\mbox{\boldmath{$\theta$}}}}
\newcommand{\bfxi}{\mbox{\boldmath{$\xi$}}}
%
\newcommand{\bfa}{{\bf a}}
\newcommand{\bfb}{{\bf b}}
\newcommand{\bfc}{{\bf c}}
\newcommand{\bfd}{{\bf d}}
\newcommand{\bfe}{{\bf e}}
\newcommand{\bff}{{\bf f}}
\newcommand{\bfg}{{\bf g}}
\newcommand{\bfh}{{\bf h}}
\newcommand{\bfk}{{\bf k}}
\newcommand{\bfl}{{\bf l}}
\newcommand{\bfht}{{\tilde{\bf h}}}
\newcommand{\bfhkl}{{\bf h}_{k+1}}
\newcommand{\bfi}{{\bf i}}
\newcommand{\bfn}{{\bf n}}
\newcommand{\bone}{{\bf 1}}
\newcommand{\bfp}{{\bf p}}
\newcommand{\bfr}{{\bf r}}
\newcommand{\bfs}{{\bf s}}
\newcommand{\bfsh}{{\hat{\bfs}}}
\newcommand{\bfst}{{\tilde{\bf s}}}
\newcommand{\bft}{{\bf t}}
\newcommand{\bfu}{{\bf u}}
\newcommand{\bfut}{{\tilde{\bf u}}}
\newcommand{\bfv}{{\bf v}}
\newcommand{\bfx}{{\bf x}}
\newcommand{\bfxt}{{\tilde{\bf x}}}
\newcommand{\bfw}{{\bf w}}
\newcommand{\bfwt}{{\tilde{\bf w}}}
\newcommand{\bfy}{{\bf y}}
\newcommand{\bfY}{{\bf Y}}
\newcommand{\bfyt}{{\tilde{\bf y}}}
\newcommand{\bfz}{{\bf z}}
\newcommand{\bfZ}{{\bf Z}}
\newcommand{\bfzt}{{\tilde{\bf z}}}
\newcommand{\bfzo}{{\bf 0}}
%
\newcommand{\bfA}{{\bf A}}
\newcommand{\bfB}{{\bf B}}
\newcommand{\bfC}{{\bf C}}
\newcommand{\C}{{\bf C}}
\newcommand{\CI}{{\bf C}^{-1}}
\newcommand{\Cbfth}{{\bf C}(\bfth)}
\newcommand{\CIbfth}{{\bf C}^{-1}(\bfth)}
\newcommand{\bfD}{{\bf D}}
\newcommand{\D}{{\bf D}}
\newcommand{\bfEk}{{\bf E}_k}
\newcommand{\bfE}{{\bf E}}
\newcommand{\bfF}{{\bf F}}
\newcommand{\bfDk}{{\bf D}_k}
\newcommand{\bfG}{{\bf G}}
\newcommand{\bfH}{{\bf H}}
\newcommand{\bfHk}{{\bf H}_k}
\newcommand{\bfI}{{\bf I}}
\newcommand{\bfJ}{{\bf J}}
\newcommand{\I}{{\bf I}(\bfth)}
\newcommand{\II}{{\bf I}^{-1}(\bfth)}
\newcommand{\bfK}{{\bf K}}
\newcommand{\bfM}{{\bf M}}
\newcommand{\bfN}{{\bf N}}
\newcommand{\bfP}{{\bf P}}
\newcommand{\bfPkp}{{\bf P}_k^\bot}
\newcommand{\bfPk}{{\bf P}_k}
\newcommand{\bfQ}{{\bf Q}}
\newcommand{\bfR}{{\bf R}}
\newcommand{\bfS}{{\bf S}}
\newcommand{\bfT}{{\bf T}}
\newcommand{\bfU}{{\bf U}}
\newcommand{\V}{{\bf V}}
\newcommand{\bfV}{{\bf V}}
\newcommand{\bfW}{{\bf W}}
\newcommand{\bfX}{{\bf X}}

